When Do LLMs Apply the Wrong Law? Diagnosing LLM Failures in Temporal Legal Reasoning

Legal reasoning requires identifying which version of a statute applies to a case, typically based on when the legally relevant events occurred rather than when the case is adjudicated. Yet whether large language models (LLMs) can reliably perform such temporal legal reasoning remains largely unexplored. We formalize this task as Temporal Applicable-Law Determination (TALD), and construct a TALD-Bench, a benchmark of 51,956 Chinese civil judgments spanning the enactment of the Civil Code. Evaluating nine advanced LLMs, we identify three key findings. First, models exhibit a strong bias toward newer law, achieving over 70% accuracy on new-law cases but below 25% on old-law cases. Second, models demonstrate substantial knowledge of statutory versions and temporal-effect rules, yet struggle to apply this knowledge to cases. Stronger general reasoning performance does not consistently translate into better TALD accuracy, whereas temporal-law hints yield substantial improvements, suggesting a bottleneck in how models deploy their existing capabilities. Third, temporal-law hints also increase uncertainty during statutory-version reasoning, suggesting that they may help models reconsider their default preference for newer law. Our findings highlight the importance of adapting how LLMs apply existing capabilities, rather than relying solely on improvements in legal knowledge or general reasoning.

==> Sections/Preliminaries.tex <==
\section{Preliminary}

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.7\linewidth]{illustration of law revision.png}
  \caption{Illustration of two typical ways of law revision, and correspondingly produced law versions.}
  \label{fig:versions}
\end{figure*}

\subsection{Temporal Versions of Statutory Law}

In legal systems where written statutes and codes play a central role, legal rules are repeatedly amended, repealed, replaced, or reorganized into new codes. As a result, the same legal issue may be regulated by multiple temporally distinct versions of law. Typically,a statute may keep the same title while individual articles are amended across years, or several previously separate statutes may be consolidated into a unified code. In such cases, different legal versions may be semantically related while only one of them is legally applicable to a particular dispute.

For the applicability of law versions, A basic default principle is non-retroactivity: newly enacted law generally does not govern legal facts or legal relationships completed before the new law took effect; while there are also legilated exceptions to this principle for purposes such as better protecting involved parties' benefit. Challenginly, real cases often cover a time span that witnesses multiple versions of an involved law. For example, a legal relationship may be formed under one statute, disputed after another statute takes effect, and adjudicated after a later code is enacted. The applicable version of an applied law therefore depends on the focal legal issue, the timing of legally relevant facts, the effective periods of candidate laws, and transitional or retroactivity rules.

Determining the correct version therefore demands professional reasoning about the temporal scope of the operative facts and the applicable inter-temporal doctrine, which is built upon the knowledge law versions together with the comprehension of legal dispute and relationships.

\subsection{Reasoning and Law Version Determination}

As a prominent recent development in LLM research, reasoning models are achieving state-of-the-art results across a broad range of tasks that require high reasoning ability. These models are further trained with reinforcement learning (RL) on verifiable tasks to produce an explicit chain-of-thought (CoT) before giving a final answer \citep{guo2025deepseek, xu2025toward}. However, tasks of reasoning-oriented RL training are predominantly limited to mathematics, formal logic, and competitive programming, which are structurally remote from many other domains that could be represented by legal reasoning, which requires navigating long natural-language texts, domain-specific principles, and context-sensitive expert judgment \citep{ma2026general, cheng2026revisiting}.

Whether reasoning capabilities acquired from such training can generalize to legal reasoning is, therefore, an open and practically important question. Law Version Determination offers a useful testbed for studying this question. From an evaluation standpoint, unlike many legal reasoning tasks whose assessment is subjective or requires costly expert annotation, the version of law applicable to a given case is uniquely determined by statute and fact, making the outcome objectively verifiable and well-suited for probing model reasoning quality at scale. From a legal reasoning standpoint, Law Version Determination is the minimum condition for of legally grounded QA, as determining the correct law article (which is versional) is a prerequisite for any further steps on analyzing and solving a legal case, making its failure a critical gap that must be understood and addressed.


==> Sections/Task_Formulation_and_Dataset.tex <==

\section{The Temporal Applicable-Law Determination Task}
\label{sec:task_dataset}


\subsection{Preliminary}
%In legal systems where written statutes and codes play a central role, legal rules are repeatedly amended, repealed, replaced, or reorganized into new codes. 
Statutory laws are repeatedly amended, repealed, replaced, or reorganized into new codes.
As a result, the same legal issue may be regulated by multiple temporally distinct versions of law. Typically,a statute may keep the same title while individual articles are amended across years, or several previously separate statutes may be consolidated into a unified code. In such cases, different legal versions may be semantically related while only one of them is legally applicable to a %particular dispute.
legal dispute.

For the applicability of law versions, A basic default principle is non-retroactivity: newly enacted law generally does not govern legal facts or legal relationships completed before the new law took effect; while there are also legilated exceptions to this principle for purposes such as better protecting involved parties' benefit. Challenginly, real cases often cover a time span that witnesses multiple versions of an 
%involved 
related
law. For example, a legal relationship may be formed under one statute, disputed after another statute takes effect, and adjudicated after a later code is enacted. The applicable version of an applied law therefore depends on the focal legal issue, the timing of legally relevant facts, the effective periods of candidate laws, and transitional or retroactivity rules.

Determining the correct version therefore demands professional reasoning about the temporal scope of the %operative facts 
case facts, locating them against the effective periods of candidate law versions, and applying temporal-effect rules
%and the applicable inter-temporal doctrine, 
and the process is built upon the knowledge law versions together with the comprehension of legal dispute and relationships.

\subsection{Task Definition}
\label{ssec:task_definition}

We formulate \textsc{Law Version Determination} (LVD) as an open-ended legal citation task. Given the facts of a case, a model is asked to suggest the laws and articles that should be applied. We use this formulation because legal cases usually involve multiple applicable laws and articles, thus the model will need to identify them and recall their versional situation, which is realistic to the application of versional law in legal QA cases.

let $x$ denote the factual narrative of a case. The model outputs a set of predicted law--article pairs:
\begin{equation}
    \hat{Y} = \{(\hat{l}_1, \hat{A}_1), \ldots, (\hat{l}_n, \hat{A}_n)\},
\end{equation}
where $\hat{l}_i$ denotes a predicted law (with version noted) and $\hat{A}_i$ denotes a set of predicted article numbers under that law. The gold citation set is:
\begin{equation}
    Y = \{(l_1, A_1), \ldots, (l_m, A_m)\}.
\end{equation}

Among the gold laws, we denote a law with possible version confusion as a \textbf{sensitive law} $l_s$, which has a known predecessor--successor relationship with another law version. We focus on testing whether the model selects the correct version of the sensitive law and the corresponding applicable articles, as respectively as coase-grained and fine-grained evidence of model's LVD capability.



==> Sections/new_split_tald_table.tex <==
\begin{table}[t]
\centering
\caption{TALD macro accuracy under the updated active-slot metric. Values are mean (standard error) across seeds.}
\label{tab:tald_updated}
\begin{tabular}{llccc}
\toprule
\textbf{Model} & \textbf{Mode} & \textbf{No hint} & \textbf{Weak hint} & \textbf{Strong hint} \\
\midrule
\multirow{2}{*}{GLM-4.7} & instruct & 0.842 (0.016) & -- & -- \
 & thinking & 0.787 (0.015) & -- & -- \
\midrule
\multirow{2}{*}{DeepSeek} & chat & 0.791 (0.015) & -- & -- \
 & reasoner & 0.746 (0.015) & -- & -- \
\midrule
\multirow{4}{*}{GPT-5.2} & none & 0.768 (0.017) & -- & -- \
 & low & 0.773 (0.007) & -- & -- \
 & medium & 0.723 (0.016) & -- & -- \
 & high & 0.719 (0.015) & -- & -- \
\midrule
\multirow{2}{*}{Qwen3-235B} & instruct & 0.761 (0.025) & -- & -- \
 & thinking & 0.730 (0.029) & -- & -- \
\midrule
\multirow{2}{*}{Qwen3-80B} & instruct & 0.619 (0.004) & -- & -- \
 & thinking & 0.798 (0.013) & -- & -- \
\midrule
\multirow{2}{*}{Qwen3-30B} & instruct & 0.336 (0.025) & -- & -- \
 & thinking & 0.765 (0.015) & -- & -- \
\midrule
\multirow{3}{*}{GPT-OSS-20B} & low & 0.437 (0.010) & -- & -- \
 & medium & 0.621 (0.029) & -- & -- \
 & high & 0.653 (0.007) & -- & -- \
\bottomrule
\end{tabular}
\end{table}


==> Sections/old_split_close_source_tald_table.tex <==
\begin{table}[t]
\centering
\caption{TALD macro accuracy under the updated active-slot metric. Values are mean (standard error) across seeds.}
\label{tab:tald_updated}
\begin{tabular}{llccc}
\toprule
\textbf{Model} & \textbf{Mode} & \textbf{No hint} & \textbf{Weak hint} & \textbf{Strong hint} \\
\midrule
\multirow{2}{*}{GLM-4.7} & instruct & 0.013 (0.007) & 0.032 (0.005) & 0.053 (0.008) \\
 & thinking & 0.080 (0.024) & 0.337 (0.019) & 0.435 (0.027) \\
\midrule
\multirow{2}{*}{DeepSeek} & chat & 0.013 (0.003) & 0.028 (0.005) & 0.080 (0.010) \\
 & reasoner & 0.092 (0.017) & 0.394 (0.013) & 0.436 (0.022) \\
\midrule
\multirow{4}{*}{GPT-5.2} & none & 0.004 (0.003) & 0.090 (0.010) & 0.191 (0.009) \\
 & low & 0.033 (0.005) & 0.369 (0.018) & 0.440 (0.025) \\
 & medium & 0.084 (0.014) & 0.290 (0.098) & 0.439 (0.026) \\
 & high & 0.094 (0.014) & 0.322 (0.107) & 0.430 (0.018) \\
\midrule
\multirow{2}{*}{Qwen3-235B} & instruct & 0.035 (0.005) & 0.035 (0.008) & 0.041 (0.009) \\
 & thinking & 0.148 (0.017) & 0.330 (0.010) & 0.323 (0.010) \\
\midrule
\multirow{2}{*}{Qwen3-80B} & instruct & 0.080 (0.006) & 0.078 (0.001) & 0.066 (0.004) \\
 & thinking & 0.028 (0.005) & 0.386 (0.006) & 0.512 (0.016) \\
\midrule
\multirow{2}{*}{Qwen3-30B} & instruct & 0.292 (0.008) & 0.264 (0.024) & 0.164 (0.013) \\
 & thinking & 0.020 (0.008) & 0.350 (0.009) & 0.395 (0.015) \\
\midrule
\multirow{3}{*}{GPT-OSS-20B} & low & 0.073 (0.017) & 0.057 (0.003) & 0.068 (0.006) \\
 & medium & 0.016 (0.005) & 0.026 (0.009) & 0.062 (0.007) \\
 & high & 0.073 (0.015) & 0.092 (0.007) & 0.101 (0.016) \\
\midrule
GLM-4.7 & default & 0.037 (0.029) & -- & -- \\
\bottomrule
\end{tabular}
\end{table}


==> Sections/old_split_opensource_tald_table.tex <==
\begin{table}[t]
\centering
\caption{TALD macro accuracy under the updated active-slot metric. Values are mean (standard error) across seeds.}
\label{tab:tald_updated}
\begin{tabular}{llccc}
\toprule
\textbf{Model} & \textbf{Mode} & \textbf{No hint} & \textbf{Weak hint} & \textbf{Strong hint} \\
\midrule
Qwen3-80B & thinking & 0.050 (0.002) & 0.459 (0.022) & 0.578 (0.024) \
\midrule
Qwen3-30B & thinking & 0.020 (0.015) & 0.371 (0.015) & 0.450 (0.020) \
\midrule
\multirow{3}{*}{GPT-OSS-20B} & low & 0.187 (0.008) & 0.172 (0.010) & 0.151 (0.030) \
 & medium & 0.073 (0.012) & 0.074 (0.007) & 0.063 (0.009) \
 & high & 0.136 (0.000) & 0.123 (0.024) & 0.147 (0.013) \
\midrule
DeepSeek-R1-Distill-Llama-70B & reasoner & 0.326 (0.025) & 0.310 (0.032) & 0.257 (0.044) \
\midrule
Llama-3.3-70B & instruct & 0.265 (0.001) & 0.252 (0.005) & 0.199 (0.015) \
\midrule
LegalOne-8B & default & 0.093 (0.008) & 0.280 (0.032) & 0.298 (0.011) \
\bottomrule
\end{tabular}
\end{table}


==> Sections/reasoning_correlations_v2.tex <==
% Generated by others/plot_reasoning_correlations.py.
\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{figures/hint_alignment_all_matched.pdf}
\caption{General reasoning benchmarks and old-law TALD accuracy. (a) No-hint correlations among GPQA, HLE, LiveCodeBench (LCB), and TALD. (b) Correlations with TALD under no, weak, and strong hints. All values are Spearman's $\rho$. External scores are fixed; TALD means are from Table~\ref{tab:default_reasoning}. Appendix~\ref{app:reasoning_benchmarks} details score sources and configuration matching.}
\label{fig:reasoning_correlations}
\end{figure*}


==> figures/app_default_prompt.tex <==
\begin{figure*}[!tp]
\centering
\fbox{\begin{minipage}{0.95\textwidth}
\small
\textbf{System: No hint}\par
You are a helpful assistant.
\medskip\par
\textbf{User: TALD}\par
If you encounter the following legal case, which legal provisions
should apply? Please respond in the format ``The applicable provisions
are Articles X, X, X of [XXX]; Articles Y, Y, Y of [YYY]; and Articles
O, O, O of [OOO].'' Write the full names of the laws, such as the
[XXX] Law of the People's Republic of China. The case is as follows:
\texttt{\{case\_facts\}\{plaintiff\_claims\}}
\end{minipage}}
\caption{TALD prompt under the no-hint condition. The user prompt is
shared across all three hint conditions.}
\label{fig:app_default_prompt}
\end{figure*}


==> figures/app_hint_prompts.tex <==
\begin{figure*}[!tp]
\centering
\fbox{\begin{minipage}{0.95\textwidth}
\small
\textbf{System: Weak temporal-law hint}\par
You are a helpful assistant. Users may ask you legal consultation
questions; please try to answer them factually. Pay attention to the
timing of events in the case and to the temporal effect of the law.
Pay attention to issues of retroactivity.
\medskip\par
\textbf{System: Strong temporal-law hint}\par
You are a helpful assistant. Users may ask you legal consultation
questions; please try to answer them factually. Pay attention to the
timing of events in the case and to the temporal effect of the law.
Pay attention to issues of retroactivity. The basic principle governing
the temporal effect of civil law is non-retroactivity, so particular
attention should be paid to whether the timing of the case facts
requires applying the old law. There are, however, exceptions, such as
beneficial retroactivity (where this better protects the lawful rights
and interests of civil subjects), retroactivity of newly introduced
provisions (where the old law had no provision and the new law adds
one), and circumstances in which newly introduced specific provisions
may be used in judicial reasoning.
\end{minipage}}
\caption{System prompts for the weak- and strong-hint conditions.}
\label{fig:app_hint_prompts}
\end{figure*}


==> figures/app_probe_prompts.tex <==
\begin{figure*}[!tp]
\centering
\fbox{\begin{minipage}{0.95\textwidth}
\small
\textbf{System: Temporal-effect rule probe}\par
You are taking a single-choice test on the temporal-effect rules of
Chinese civil substantive law. Based on the question, recall the
general principles governing the temporal effect of civil law and
the Provisions of the Supreme People's Court on the Temporal Effect
of the Application of the Civil Code of the People's Republic of
China, and choose the most appropriate answer. Your final response
must contain only one available uppercase option letter, such as
A or B. Do not explain your reasoning or output any other text.
\medskip\par
\textbf{User: Temporal-effect rule probe}\par
Condition: \texttt{\{condition\}}\par
Question: \texttt{\{question\}}\par
Options:\par
A. \texttt{\{choices[A]\}}\par
B. \texttt{\{choices[B]\}}\par
Output only the letter of the correct option.

\medskip\hrule\medskip
\textbf{Examples from the fixed question set}\par
\textit{Question (both examples).} Which rules of substantive civil
law should apply?\par
\textit{Options (both examples).} A. The Civil Code or its relevant
provisions (new law); B. The laws and judicial interpretations in
force at the relevant earlier time (old law).
\smallskip\par
\textit{General rule (Article~1(2)).} A civil dispute arises from
legal facts occurring before the Civil Code takes effect, with no
exception specified by a law or judicial interpretation.\par
\textit{Correct answer.} B.
\smallskip\par
\textit{Transitional rule (Article~20).} A contract was formed before
the Civil Code took effect, and performance continues afterwards by
law or agreement. The dispute concerns performance occurring after
the Code took effect.\par
\textit{Correct answer.} A.
\end{minipage}}
\caption{English translations of the temporal-effect rule prompt
and two example questions. Source provisions refer to the judicial
interpretation. Answers and source-article references are shown for
illustration and are not included in the model input.}
\label{fig:app_probe_prompts}
\end{figure*}


==> figures/app_version_probe.tex <==
\begin{figure*}[!t]
\centering
\fbox{\begin{minipage}{0.95\textwidth}
\small
\textbf{Prompt: statutory-version knowledge}\par
\textit{System.} You are taking a multiple-choice test on knowledge
of old and new versions of Chinese substantive civil law. You will
see the original text of a legal provision and two possible statutory
versions. Identify which version the provision comes from. Your
final answer must contain only one available uppercase option letter,
such as A or B. Do not explain your reasoning or output any other text.
\medskip\par
\textit{User.} Below is the original text of a provision of Chinese
substantive civil law. Identify which statutory version it comes from.\par
Provision: \texttt{\{article\_text\}}\par
Options: A. \texttt{\{choices[A]\}}; B. \texttt{\{choices[B]\}}\par
Output only the uppercase letter of the correct option, such as A
or B. Do not explain.
\medskip\hrule\medskip
\textbf{Example from the fixed question set}\par
\textit{Provision.} Where a child of the deceased dies before the
deceased, the child's direct lineal descendants inherit by
representation. A successor by representation generally inherits
only the share to which their father or mother would have been entitled.\par
\textit{Options.} A. Civil Code of the People's Republic of China,
Book VI: Succession; B. Succession Law of the People's Republic of China.\par
\textit{Correct answer.} B.
\end{minipage}}
\caption{English translations of the statutory-version prompt and
one old-law question. The answer is shown for illustration and is
not included in the model input.}
\label{fig:app_version_probe}
\end{figure*}


==> figures/reasoning_correlations.tex <==
% Generated by others/plot_reasoning_correlations.py.
\begin{figure*}[t]
\centering
\captionsetup[subfloat]{position=top,font={small,sf,bf}}
\definecolor{reasoning0}{HTML}{245F9E}
\definecolor{reasoning1}{HTML}{897675}
\definecolor{reasoning2}{HTML}{B92E26}
\definecolor{reasoning3}{HTML}{5B7B99}
\definecolor{reasoning4}{HTML}{5096DE}
\definecolor{reasoning5}{HTML}{32485E}
\definecolor{reasoning6}{HTML}{A6C8EA}
\subfloat[GPQA and TALD.\label{fig:gpqa_tald}]{%
\begin{minipage}[t]{0.32\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
tald plot,
width=0.69\linewidth, height=3.5cm, scale only axis,
axis lines*=left, axis line style={taldaxis, line width=0.6pt}, tick style={taldaxis},
tick align=outside, tick label style={font=\scriptsize\sffamily},
label style={font=\small\sffamily}, ymajorgrids=true, grid style={taldgrid, line width=0.5pt},
xlabel={GPQA score}, ylabel={TALD accuracy},
xmin=62, xmax=93, xtick={65,75,85},
ymin=0, ymax=0.33, ytick={0,0.1,0.2,0.3},
legend to name=reasoninglegend, legend columns=4,
legend style={draw=none,font=\scriptsize\sffamily,/tikz/every even column/.append style={column sep=1em}},
]
\addplot[only marks, color=reasoning0, mark=o, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(75.1,0.013)};
\addplot[only marks, color=reasoning0, mark=*, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(84,0.092)};
\addlegendimage{only marks,color=reasoning0,mark=*}
\addlegendentry{DeepSeek-V3.2}
\addplot[only marks, color=reasoning1, mark=*, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(89.6,0.014)};
\addlegendimage{only marks,color=reasoning1,mark=*}
\addlegendentry{Claude Opus 4.6}
\addplot[only marks, color=reasoning2, mark=o, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(74.8,0.021)};
\addplot[only marks, color=reasoning2, mark=*, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(87.1,0.082)};
\addlegendimage{only marks,color=reasoning2,mark=*}
\addlegendentry{GPT-5.4}
\addplot[only marks, color=reasoning3, mark=o, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(66.4,0.013)};
\addplot[only marks, color=reasoning3, mark=*, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(85.9,0.08)};
\addlegendimage{only marks,color=reasoning3,mark=*}
\addlegendentry{GLM-4.7}
\addplot[only marks, color=reasoning4, mark=o, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(75.3,0.035)};
\addplot[only marks, color=reasoning4, mark=*, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(79,0.148)};
\addlegendimage{only marks,color=reasoning4,mark=*}
\addlegendentry{Qwen3-235B}
\addplot[only marks, color=reasoning5, mark=o, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(73.8,0.08)};
\addplot[only marks, color=reasoning5, mark=*, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(75.9,0.028)};
\addlegendimage{only marks,color=reasoning5,mark=*}
\addlegendentry{Qwen3-80B}
\addplot[only marks, color=reasoning6, mark=o, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(65.9,0.292)};
\addplot[only marks, color=reasoning6, mark=*, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(70.7,0.02)};
\addlegendimage{only marks,color=reasoning6,mark=*}
\addlegendentry{Qwen3-30B}
\node[anchor=north east,font=\small\sffamily\bfseries\boldmath,align=left,fill=white,inner sep=2pt] at (rel axis cs:0.97,0.98) {$\rho=0.15$};
\end{axis}
\end{tikzpicture}
\end{minipage}}
\hfill
\subfloat[HLE and TALD.\label{fig:hle_tald}]{%
\begin{minipage}[t]{0.32\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
tald plot,
width=0.69\linewidth, height=3.5cm, scale only axis,
axis lines*=left, axis line style={taldaxis, line width=0.6pt}, tick style={taldaxis},
tick align=outside, tick label style={font=\scriptsize\sffamily},
label style={font=\small\sffamily}, ymajorgrids=true, grid style={taldgrid, line width=0.5pt},
xlabel={HLE score}, ylabel={TALD accuracy},
xmin=0, xmax=44, xtick={0,20,40},
ymin=0, ymax=0.33, ytick={0,0.1,0.2,0.3},
]
\addplot[only marks, color=reasoning0, mark=o, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(11.2,0.013)};
\addplot[only marks, color=reasoning0, mark=*, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(24.6,0.092)};
\addplot[only marks, color=reasoning1, mark=*, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(39.9,0.014)};
\addplot[only marks, color=reasoning2, mark=o, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(11.3,0.021)};
\addplot[only marks, color=reasoning2, mark=*, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(30.8,0.082)};
\addplot[only marks, color=reasoning3, mark=o, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(6.4,0.013)};
\addplot[only marks, color=reasoning3, mark=*, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(27.4,0.08)};
\addplot[only marks, color=reasoning4, mark=o, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(11.1,0.035)};
\addplot[only marks, color=reasoning4, mark=*, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(15.9,0.148)};
\addplot[only marks, color=reasoning5, mark=o, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(7.6,0.08)};
\addplot[only marks, color=reasoning5, mark=*, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(12.6,0.028)};
\addplot[only marks, color=reasoning6, mark=o, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(6.9,0.292)};
\addplot[only marks, color=reasoning6, mark=*, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(10.3,0.02)};
\node[anchor=north east,font=\small\sffamily\bfseries\boldmath,align=left,fill=white,inner sep=2pt] at (rel axis cs:0.97,0.98) {$\rho=0.16$};
\end{axis}
\end{tikzpicture}
\end{minipage}}
\hfill
\subfloat[GPQA and HLE.\label{fig:gpqa_hle}]{%
\begin{minipage}[t]{0.32\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
tald plot,
width=0.69\linewidth, height=3.5cm, scale only axis,
axis lines*=left, axis line style={taldaxis, line width=0.6pt}, tick style={taldaxis},
tick align=outside, tick label style={font=\scriptsize\sffamily},
label style={font=\small\sffamily}, ymajorgrids=true, grid style={taldgrid, line width=0.5pt},
xlabel={GPQA score}, ylabel={HLE score},
xmin=62, xmax=93, xtick={65,75,85},
ymin=0, ymax=44, ytick={0,20,40},
]
\addplot[only marks, color=reasoning0, mark=o, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(75.1,11.2)};
\addplot[only marks, color=reasoning0, mark=*, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(84,24.6)};
\addplot[only marks, color=reasoning1, mark=*, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(89.6,39.9)};
\addplot[only marks, color=reasoning2, mark=o, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(74.8,11.3)};
\addplot[only marks, color=reasoning2, mark=*, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(87.1,30.8)};
\addplot[only marks, color=reasoning3, mark=o, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(66.4,6.4)};
\addplot[only marks, color=reasoning3, mark=*, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(85.9,27.4)};
\addplot[only marks, color=reasoning4, mark=o, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(75.3,11.1)};
\addplot[only marks, color=reasoning4, mark=*, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(79,15.9)};
\addplot[only marks, color=reasoning5, mark=o, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(73.8,7.6)};
\addplot[only marks, color=reasoning5, mark=*, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(75.9,12.6)};
\addplot[only marks, color=reasoning6, mark=o, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(65.9,6.9)};
\addplot[only marks, color=reasoning6, mark=*, mark size=2.5pt, line width=0.85pt, forget plot] coordinates {(70.7,10.3)};
\node[anchor=north west,font=\small\sffamily\bfseries\boldmath,align=left,fill=white,inner sep=2pt] at (rel axis cs:0.03,0.98) {$\rho=0.97$};
\end{axis}
\end{tikzpicture}
\end{minipage}}
\par\vspace{0.4em}
\pgfplotslegendfromname{reasoninglegend}
\caption{Correlations across 13 matched model configurations. External scores are on a 0--100 scale; TALD accuracy is on old-law cases under the default instruction. Colors identify models. Open circles denote chat, instruct, or no-effort configurations; filled circles denote reasoner, thinking, Claude max, or GPT low-effort configurations. $\rho$ is Spearman's rank correlation.}
\label{fig:reasoning_correlations}
\end{figure*}


==> others/TALD_main_references.tex <==
% Generated from main.aux; rerun others/refresh_preview_refs.py after compiling the manuscript.
\newlabel{ssec:rq2_knowledge}{{4.2}{4}{}{}{}}
\newlabel{fig:fault_types}{{2b}{5}{}{}{}}
\newlabel{ssec:rq3_setup}{{4.3}{7}{}{}{}}
\newlabel{sssec:rq2_hint}{{4.2}{6}{}{}{}}
\newlabel{sssec:rq2_general_reasoning}{{4.2}{5}{}{}{}}
\newlabel{fig:reasoning_correlations}{{4}{6}{}{}{}}
\newlabel{tab:default_reasoning}{{1}{6}{}{}{}}
\newlabel{fig:rq1_initial}{{2a}{5}{}{}{}}
\newlabel{fig:rq3_main}{{5}{7}{}{}{}}


==> savespace.tex <==
\usepackage[all=normal, floats, bibnotes, wordspacing, charwidths, indent]{savetrees}

\makeatletter%
%
\skip\footins 8.1pt plus 4pt minus 2pt % Space between last line of text top
                                      % and of first footnote.
\floatsep 5pt plus 2pt minus 2pt        % Space between adjacent floats moved
                                         % to top or bottom of text page.
\textfloatsep 5pt plus 2pt minus 4pt    % Space between main text and floats
                                         % at top or bottom of page.
\intextsep 5pt plus 2pt minus 2pt       % Space between in-text figures and
                                         % text.
%\@maxsep 5pt                            % The maximum of \floatsep,
                                         % \textfloatsep and \intextsep (minus
                                         % the stretch and shrink).
\dblfloatsep 5pt plus 0pt minus 0pt     % Same as \floatsep for double-column
                                         % figures in two-column mode.
\dbltextfloatsep 5pt plus 0pt minus 0pt % \textfloatsep for double-column
                                         % floats.
%\@dblmaxsep 5pt                         % The maximum of \dblfloatsep and
                                         % \dbltexfloatsep.

==> tables/app_external_reasoning.tex <==
\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}llrrrrr@{}}
\toprule
\textbf{Model} & \textbf{Mode} & \textbf{GPQA} & \textbf{HLE} & \textbf{AIME~2025} & \textbf{LiveCodeBench} & \textbf{TALD} \\
\midrule
DeepSeek-V3.2 & chat & 75.1 & 11.2 & 59.0 & 59.3 & 0.013 \\
 & reasoner & 84.0 & 24.6 & 92.0 & 86.2 & 0.092 \\
\addlinespace[3pt]
Claude Opus 4.6 & max & 89.6 & 39.9 & -- & -- & 0.014 \\
\addlinespace[3pt]
GPT-5.4 & none & 74.8 & 11.3 & -- & -- & 0.021 \\
 & low & 87.1 & 30.8 & -- & -- & 0.082 \\
\addlinespace[3pt]
GLM-4.7 & instruct & 66.4 & 6.4 & 48.0 & 56.2 & 0.013 \\
 & thinking & 85.9 & 27.4 & 95.0 & 89.4 & 0.080 \\
\addlinespace[3pt]
Qwen3-235B & instruct & 75.3 & 11.1 & 71.7 & 52.4 & 0.035 \\
 & thinking & 79.0 & 15.9 & 91.0 & 78.8 & 0.148 \\
\addlinespace[3pt]
Qwen3-80B & instruct & 73.8 & 7.6 & 66.3 & 68.4 & 0.080 \\
 & thinking & 75.9 & 12.6 & 84.3 & 78.4 & 0.028 \\
\addlinespace[3pt]
Qwen3-30B & instruct & 65.9 & 6.9 & 66.3 & 51.5 & 0.292 \\
 & thinking & 70.7 & 10.3 & 56.3 & 70.7 & 0.020 \\
\midrule
\multicolumn{2}{l}{Matched $N$} & 13 & 13 & 10 & 10 & \\
\multicolumn{2}{l}{Spearman $\rho$} & 0.15 & 0.16 & 0.62 & 0.19 & \\
\bottomrule
\end{tabular*}
\caption{Artificial Analysis scores (0--100) and default TALD accuracy on old-law cases (0--1). $N$ counts matched configurations; dashes indicate unavailable scores.}
\label{tab:app_external_reasoning}
\end{table*}


==> tables/app_external_reasoning_v2.tex <==
% External score columns are source data; TALD columns and footer are refreshed
% from tables/default_reasoning.tex by others/plot_reasoning_correlations.py.
\begin{table*}[t]
\centering
\begingroup\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}llrrrrrr@{}}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Mode}} & \multicolumn{3}{c}{\textbf{External benchmark score}} & \multicolumn{3}{c}{\textbf{Old-law TALD accuracy}} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}
 & & \textbf{GPQA} & \textbf{HLE} & \textbf{LCB} & \textbf{No hint} & \textbf{Weak hint} & \textbf{Strong hint} \\
\midrule
DeepSeek-V3.2 & chat & 75.1 & 11.2 & 59.3 & 0.013 & 0.028 & 0.080 \\
 & reasoner & 84.0 & 24.6 & 86.2 & 0.092 & 0.394 & 0.436 \\
\addlinespace[3pt]
Claude Opus 4.6 & max & 89.6 & 39.9 & -- & 0.014 & 0.113 & 0.156 \\
\addlinespace[3pt]
GPT-5.4 & none & 74.8 & 11.3 & -- & 0.021 & 0.087 & 0.167 \\
 & low & 87.1 & 30.8 & -- & 0.082 & 0.444 & 0.456 \\
\addlinespace[3pt]
GLM-4.7 & instruct & 66.4 & 6.4 & 56.2 & 0.013 & 0.032 & 0.053 \\
 & thinking & 85.9 & 27.4 & 89.4 & 0.080 & 0.337 & 0.435 \\
\addlinespace[3pt]
Qwen3-235B & instruct & 75.3 & 11.1 & 52.4 & 0.035 & 0.035 & 0.041 \\
 & thinking & 79.0 & 15.9 & 78.8 & 0.148 & 0.330 & 0.323 \\
\addlinespace[3pt]
Qwen3-80B & instruct & 73.8 & 7.6 & 68.4 & 0.080 & 0.078 & 0.066 \\
 & thinking & 75.9 & 12.6 & 78.4 & 0.028 & 0.386 & 0.512 \\
\addlinespace[3pt]
Qwen3-30B & instruct & 65.9 & 6.9 & 51.5 & 0.292 & 0.264 & 0.164 \\
 & thinking & 70.7 & 10.3 & 70.7 & 0.020 & 0.350 & 0.395 \\
\midrule
\multicolumn{2}{l}{Matched $N$} & 13 & 13 & 10 &  &  &  \\
\multicolumn{2}{l}{Spearman $\rho$: No hint} & 0.146 & 0.163 & 0.189 &  &  &  \\
\multicolumn{2}{l}{Spearman $\rho$: Weak hint} & 0.467 & 0.549 & 0.697 &  &  &  \\
\multicolumn{2}{l}{Spearman $\rho$: Strong hint} & 0.456 & 0.577 & 0.758 &  &  &  \\
\bottomrule
\end{tabular*}
\endgroup
\caption{Artificial Analysis benchmark scores (0--100) and old-law TALD accuracy (0--1) under no, weak, and strong hints. TALD columns report the across-seed means from Table~\TALDMainRef{tab:default_reasoning}. The bottom rows give each benchmark's matched configuration count and Spearman correlation with TALD under each hint condition; matching is fixed across conditions. Dashes indicate unavailable scores..}
\label{tab:app_external_reasoning}
\end{table*}

==> tables/app_model_ids.tex <==
\begin{table*}[!t]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}>{\raggedright\arraybackslash}p{0.22\linewidth}>{\raggedright\arraybackslash}p{0.25\linewidth}>{\raggedright\arraybackslash}p{\dimexpr0.53\linewidth-4\tabcolsep\relax}@{}}
\toprule
\multicolumn{3}{l}{\textbf{(a) API model IDs used in evaluation}} \\
\midrule
\textbf{Name in paper} & \textbf{Mode(s) in results} & \textbf{API model ID} \\
\midrule
DeepSeek-V3.2 & chat & \texttt{deepseek-chat} \\
 & reasoner & \texttt{deepseek-reasoner} \\
\addlinespace[3pt]
GLM-4.7 & instruct; thinking & \texttt{z-ai/glm-4.7} \\
\addlinespace[3pt]
GPT-5.4 & none; low; medium; high & \texttt{gpt-5.4} \\
\addlinespace[3pt]
Gemini-3.1-Pro & low; medium; high & \texttt{gemini-3.1-pro-preview} \\
\addlinespace[3pt]
Claude Opus 4.6 & low; medium; high; max & \texttt{claude-opus-4-6} \\
\bottomrule
\end{tabular*}\par\vspace{8pt}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}>{\raggedright\arraybackslash}p{0.22\linewidth}>{\raggedright\arraybackslash}p{0.25\linewidth}>{\raggedright\arraybackslash}p{\dimexpr0.53\linewidth-4\tabcolsep\relax}@{}}
\toprule
\multicolumn{3}{l}{\textbf{(b) Open-weight model repositories}} \\
\midrule
\textbf{Name in paper} & \textbf{Mode in results} & \textbf{Hugging Face repository} \\
\midrule
Qwen3-235B & instruct & \href{https://huggingface.co/Qwen/Qwen3-235B-A22B-Instruct-2507}{\texttt{Qwen/Qwen3-235B-A22B-Instruct-2507}} \\
 & thinking & \href{https://huggingface.co/Qwen/Qwen3-235B-A22B-Thinking-2507}{\texttt{Qwen/Qwen3-235B-A22B-Thinking-2507}} \\
\addlinespace[3pt]
Qwen3-80B & instruct & \href{https://huggingface.co/Qwen/Qwen3-Next-80B-A3B-Instruct}{\texttt{Qwen/Qwen3-Next-80B-A3B-Instruct}} \\
 & thinking & \href{https://huggingface.co/Qwen/Qwen3-Next-80B-A3B-Thinking}{\texttt{Qwen/Qwen3-Next-80B-A3B-Thinking}} \\
\addlinespace[3pt]
Qwen3-30B & instruct & \href{https://huggingface.co/Qwen/Qwen3-30B-A3B-Instruct-2507}{\texttt{Qwen/Qwen3-30B-A3B-Instruct-2507}} \\
 & thinking & \href{https://huggingface.co/Qwen/Qwen3-30B-A3B-Thinking-2507}{\texttt{Qwen/Qwen3-30B-A3B-Thinking-2507}} \\
\addlinespace[3pt]
LegalOne-8B & reasoning & \href{https://huggingface.co/CSHaitao/LegalOne-8B}{\texttt{CSHaitao/LegalOne-8B}} \\
\bottomrule
\end{tabular*}
\caption{Names used in the paper and their corresponding evaluated
configurations. Panel (a) reports API request identifiers used
during evaluation; panel (b) links to the corresponding Hugging Face
model repositories.}
\label{tab:app_model_ids}
\label{tab:app_qwen_ids}
\end{table*}


==> tables/app_statute_families.tex <==
\begin{table*}[!tp]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}>{\raggedright\arraybackslash}p{0.21\linewidth}>{\raggedright\arraybackslash}p{0.39\linewidth}>{\raggedright\arraybackslash}p{\dimexpr0.40\linewidth-4\tabcolsep\relax}@{}}
\toprule
\textbf{Area of civil law} & \textbf{Predecessor statute(s)} & \textbf{Civil Code counterpart} \\
\midrule
General provisions & General Principles of the Civil Law; General Provisions of the Civil Law & Book I: General Provisions \\
\addlinespace[2pt]
Property & Property Law & Book II: Real Rights \\
\addlinespace[2pt]
Contract & Contract Law & Book III: Contracts \\
\addlinespace[2pt]
Personality rights & --- & Book IV: Personality Rights \\
\addlinespace[2pt]
Marriage and family & Marriage Law & Book V: Marriage and Family \\
\addlinespace[2pt]
Inheritance & Succession Law & Book VI: Succession \\
\addlinespace[2pt]
Tort liability & Tort Liability Law & Book VII: Tort Liability \\
\addlinespace[2pt]
Adoption & Adoption Law & Adoption provisions in Book V \\
\addlinespace[2pt]
Security & Security Law & Selected provisions in Books II and III \\
\bottomrule
\end{tabular*}
\caption{Predecessor statutes and their Civil Code counterparts,
grouped by area of civil law. A dash indicates that no separate
predecessor statute is listed for that area.}
\label{tab:app_statute_families}
\end{table*}


==> tables/rq3_main.tex <==
\begin{table*}[t]
\centering
\begingroup
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.7}
% Match Table 1: a full-size mean above a smaller standard error.
\newcommand{\taldresult}[2]{%
  \begingroup
  \renewcommand{\arraystretch}{0.8}%
  \begin{tabular}[c]{@{}c@{}}%
    #1\\[-2pt]%
    {\scriptsize\textpm{}\,#2}%
  \end{tabular}%
  \endgroup
}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}llcccccc@{}}
\toprule
\multirow{2}{*}[-4pt]{\textbf{Model}} & \multirow{2}{*}[-4pt]{\textbf{Mode}}
& \multicolumn{2}{c}{\textbf{No hint}}
& \multicolumn{2}{c}{\textbf{Weak hint}}
& \multicolumn{2}{c}{\textbf{Strong hint}} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
& & ACC & $H_i^{ver}$ & ACC & $H_i^{ver}$ & ACC & $H_i^{ver}$ \\
\midrule
Qwen3-235B  & thinking  & \taldresult{0.155}{0.025} & \taldresult{0.238}{0.006} & \taldresult{0.524}{0.025} & \taldresult{0.253}{0.004} & \taldresult{0.523}{0.032} & \taldresult{0.266}{0.005} \\
\specialrule{0.25pt}{1.125pt}{1.125pt}
Qwen3-80B   & thinking  & \taldresult{0.050}{0.002} & \taldresult{1.148}{0.026} & \taldresult{0.459}{0.022} & \taldresult{1.185}{0.029} & \taldresult{0.578}{0.024} & \taldresult{1.211}{0.025} \\
\specialrule{0.25pt}{1.125pt}{1.125pt}
Qwen3-30B   & thinking  & \taldresult{0.020}{0.015} & \taldresult{0.315}{0.005} & \taldresult{0.371}{0.015} & \taldresult{0.425}{0.010} & \taldresult{0.450}{0.020} & \taldresult{0.462}{0.014} \\
\specialrule{0.25pt}{1.125pt}{1.125pt}
LegalOne-8B & reasoning & \taldresult{0.093}{0.008} & \taldresult{0.147}{0.006} & \taldresult{0.280}{0.032} & \taldresult{0.159}{0.002} & \taldresult{0.298}{0.011} & \taldresult{0.173}{0.003} \\
\bottomrule
\end{tabular*}
\endgroup
\caption{
TALD accuracy and version-related policy entropy $H_i^{ver}$ on old-law cases across hint strength. Each cell shows the mean above and $\pm$ its standard error below, computed over three random seeds.
}
\label{tab:app_rq3_main}
% Preserve compatibility with the label used in the current manuscript.
\label{tab:app_rq3_mainv}
\end{table*}
